Matched Topological Subspace Detector

Topological spaces, represented by simplicial complexes, capture richer relationships than graphs by modeling interactions not only between nodes but also among higher-order entities, such as edges or triangles. This motivates the representation of information defined in irregular domains as topological signals. By leveraging the spectral dualities of Hodge and Dirac theory, practical topological signals often concentrate in specific spectral subspaces (e.g., gradient or curl). For instance, in a foreign currency exchange network, the exchange flow signals typically satisfy the arbitrage-free condition and hence are curl-free. However, the presence of anomalies can disrupt these conditions, causing the signals to deviate from such subspaces. In this work, we formulate a hypothesis testing framework to detect whether simplicial complex signals lie in specific subspaces in a principled and tractable manner. Concretely, we propose Neyman-Pearson matched topological subspace detectors for signals defined at a single simplicial level (such as edges) or jointly across all levels of a simplicial complex. The (energy-based projection) proposed detectors handle missing values, provide closed-form performance analysis, and effectively capture the unique topological properties of the data. We demonstrate the effectiveness of the proposed topological detectors on various real-world data, including foreign currency exchange networks.

==> ProofProposition2.tex <==
\subsection{Proof of Proposition \ref{prop:hodge_zero}}
\label{sub:proof_prop_zeropad}
We start by proving~\eqref{eq:hodge_zero1}. %The condition $[\boldsymbol{0}\|\boldsymbol{s}^1\| \boldsymbol{0}]\in \operatorname{span}\left(\mathbf{D}_l\right)$ indicates that there exists a nonzero simplicial signal $[\widetilde{\boldsymbol{s}}^0\|\widetilde{\boldsymbol{s}}^1\| \widetilde{\boldsymbol{s}}^2]$ that satisfies
\begin{equation}
\left[\begin{array}{c}
\mathbf{0} \\
\boldsymbol{s}^1\\
\mathbf{0} 
\end{array}\right] = \left[\begin{array}{ccc}
\mathbf{0} & \mathbf{B}_1 & \mathbf{0} \\
\mathbf{B}_1^{\top} & \mathbf{0} & \mathbf{0} \\
\mathbf{0} & \mathbf{0} & \mathbf{0}
\end{array}\right]\left[\begin{array}{c}
\widetilde{\boldsymbol{s}}^0 \\
\widetilde{\boldsymbol{s}}^1\\
\widetilde{\boldsymbol{s}}^2
\end{array}\right]=\left[\begin{array}{c}
\mathbf{B}_1\widetilde{\boldsymbol{s}}^1 \\
\mathbf{B}_1^\top\widetilde{\boldsymbol{s}}^0\\
\mathbf{0} 
\end{array}\right].
\end{equation}
This means that $\mathbf{B}_1\widetilde{\boldsymbol{s}}^1 = \mathbf{0}$ and $\boldsymbol{s}^1 = \mathbf{B}_1^\top\widetilde{\boldsymbol{s}}^0\in \operatorname{span}\left(\mathbf{B}_1^\top\right)$, which proves that $\left[\boldsymbol{0}\|\boldsymbol{s}^1\| \boldsymbol{0}\right]\in \operatorname{span}\left(\mathbf{D}_l\right)\Rightarrow \boldsymbol{s}^1 \in\operatorname{span}\left(\mathbf{B}_1^\top\right)$.

Next, we show that the converse, i.e., $\boldsymbol{s}^1 \in\operatorname{span}\left(\mathbf{B}_1^\top\right) \Rightarrow \left[\boldsymbol{0}\|\boldsymbol{s}^1\| \boldsymbol{0}\right]\in \operatorname{span}\left(\mathbf{D}_l\right)$ is also true. The condition $\boldsymbol{s}^1 \in\operatorname{span}\left(\mathbf{B}_1^\top\right)$ implies that there exists a $0-$signal $\widetilde{\boldsymbol{s}}^0$ satisfying that $\boldsymbol{s}^1 = \mathbf{B}_1^\top \widetilde{\boldsymbol{s}}^0$. We can write this as a function of $\bbD_l$ as
\begin{equation}
 \left[\begin{array}{ccc}
\mathbf{0} & \mathbf{B}_1 & \mathbf{0} \\
\mathbf{B}_1^{\top} & \mathbf{0} & \mathbf{0} \\
\mathbf{0} & \mathbf{0} & \mathbf{0}
\end{array}\right]\left[\begin{array}{c}
\widetilde{\boldsymbol{s}}^0 \\
\boldsymbol{0}\\
\boldsymbol{0}
\end{array}\right]=\left[\begin{array}{c}
\boldsymbol{0} \\
\mathbf{B}_1^\top\widetilde{\boldsymbol{s}}^0\\
\mathbf{0} 
\end{array}\right]=\left[\begin{array}{c}
\mathbf{0} \\
\boldsymbol{s}^1\\
\mathbf{0} 
\end{array}\right]
\end{equation}
which indicates that $[\boldsymbol{0}\|\boldsymbol{s}^1\| \boldsymbol{0}]\in \operatorname{span}\left(\mathbf{D}_l\right)$. The proof of $\left[\boldsymbol{0}\|\boldsymbol{s}^1\| \boldsymbol{0}\right]\in \operatorname{span}\left(\mathbf{D}_l\right)\Rightarrow \boldsymbol{s}^1 \in\operatorname{span}\left(\mathbf{B}_1^\top\right)$ completes, therefore completing the proof of~\eqref{eq:hodge_zero1}. The proof of equation~\eqref{eq:hodge_zero2} is equivalent to that of~\eqref{eq:hodge_zero1}.

The proof of equation~\eqref{eq:hodge_zero3} is provided next: the condition $\left[\boldsymbol{0}\|\boldsymbol{s}^1\| \boldsymbol{0}\right]\in \operatorname{kernel}\left(\mathbf{D}\right)$ indicates that $\mathbf{D} \left[\boldsymbol{0}\|\boldsymbol{s}^1\| \boldsymbol{0}\right] = \boldsymbol{0}$. We can multiply both sides of the equation by $\mathbf{D}$ to write $\mathbf{D}^2 \left[\boldsymbol{0}\|\boldsymbol{s}^1\| \boldsymbol{0}\right] = \mathbf{D} \boldsymbol{0} = \boldsymbol{0}$ so that we are able to use the definition of $\mathbf{D}^2$ as the block diagonal matrix with the Hodge Laplacians and write
\begin{equation}
 \left[\begin{array}{ccc}
\mathbf{L}_0 & \mathbf{0} & \mathbf{0} \\
\mathbf{0} & \mathbf{L}_1 & \mathbf{0} \\
\mathbf{0} & \mathbf{0} & \mathbf{L}_2
\end{array}\right]\left[\begin{array}{c}
\mathbf{0} \\
\boldsymbol{s}^1\\
\mathbf{0} 
\end{array}\right]=\left[\begin{array}{c}
\mathbf{0} \\
\mathbf{L}_1\boldsymbol{s}^1\\
\mathbf{0} 
\end{array}\right]=\mathbf{0} 
\end{equation}
which indicates $\mathbf{L}_1\boldsymbol{s}^1 = \mathbf{0}\Rightarrow\boldsymbol{s}^1\in \operatorname{kernel}\left(\mathbf{L}_1\right)$ and proves that $\left[\boldsymbol{0}\|\boldsymbol{s}^1\| \boldsymbol{0}\right]\in \operatorname{kernel}\left(\mathbf{D}\right) \Rightarrow \boldsymbol{s}^1\in \operatorname{kernel}\left(\mathbf{L}_1\right)$. Regarding the converse, the condition $\boldsymbol{s}^1\in \operatorname{kernel}\left(\mathbf{L}_1\right)$ indicates that $\boldsymbol{s}^1$ is a solution to $\mathbf{L}_1\boldsymbol{s}^1 = \mathbf{0}$. Considering that $\mathbf{D}$ and $\mathbf{D}^2=\mathcal{L}$ share the same kernel space (as they share eigenvectors and squaring the eigenvalues do not change which of them are 0), $\left[\boldsymbol{0}\|\boldsymbol{s}^1\| \boldsymbol{0}\right]$ lives in the kernel space of $\mathbf{D}$~\cite{calmon2022higher}, therefore proving that $\boldsymbol{s}^1\in \operatorname{kernel}\left(\mathbf{L}_1\right) \Rightarrow \left[\boldsymbol{0}\|\boldsymbol{s}^1\| \boldsymbol{0}\right]\in \operatorname{kernel}\left(\mathbf{D}\right)$. This completes the proof of equation~\eqref{eq:hodge_zero3} and therefore of Proposition~\ref{prop:hodge_zero}.
